Spanning Adjacency Oracles in Sublinear Time

Suppose we are given an $n$-node, $m$-edge input graph $G$, and the goal is to compute a spanning subgraph $H$ on $O(n)$ edges. This can be achieved in linear $O(m + n)$ time via breadth-first search. But can we hope for \emph{sublinear} runtime in some range of parameters? If the goal is to return $H$ as an adjacency list, there are simple lower bounds showing that $\Omega(m + n)$ runtime is necessary. If the goal is to return $H$ as an adjacency matrix, then we need $\Omega(n^2)$ time just to write down the entries of the output matrix. However, we show that neither of these lower bounds still apply if instead the goal is to return $H$ as an \emph{implicit} adjacency matrix, which we call an \emph{adjacency oracle}. An adjacency oracle is a data structure that gives a user the illusion that an adjacency matrix has been computed: it accepts edge queries $(u, v)$, and it returns in near-constant time a bit indicating whether $(u, v) \in E(H)$. Our main result is that one can construct an adjacency oracle for a spanning subgraph on at most $(1+\varepsilon)n$ edges, in $\tilde{O}(n \varepsilon^{-1})$ time, and that this construction time is near-optimal. Additional results include constructions of adjacency oracles for $k$-connectivity certificates and spanners, which are similarly sublinear on dense-enough input graphs. Our adjacency oracles are closely related to Local Computation Algorithms (LCAs) for graph sparsifiers; they can be viewed as LCAs with some computation moved to a preprocessing step, in order to speed up queries. Our oracles imply the first Local algorithm for computing sparse spanning subgraphs of general input graphs in $\tilde{O}(n)$ query time, which works by constructing our adjacency oracle, querying it once, and then throwing the rest of the oracle away. This addresses an open problem of Rubinfeld [CSR '17].

==> DistributedSetting.tex <==
\section{Extending to the Distributed Setting}
The idea of outputting spanning subgraphs as adjacency oracles instead of adjacency lists can be applied to other models of computation. One particularly natural setting is the \texttt{CONGEST} model of distributed computation.

The fact that adjacency oracles defer computation of the  subgraph $H$ until query time is essential to overcoming the cut-edge lower bound. In a similar vein, typical \texttt{CONGEST} model solutions are ``outputted'' in the sense of each vertex storing its subgraph adjacency list. However, another valid representation of the adjacencies of the vertex is a vertex-specific adjacency oracle. Namely, the adjacency oracle corresponding to vertex $v$ gives the illusion of having access to the $v$\textsuperscript{th} row of the adjacency matrix of $H$ by responding to queries of edges incident to $v$ in $\Oish(1)$ time, outputting whether or not the edge is in $H$.

Given that there are now $|V|$ different adjacency oracles, the consistency of our representation of $H$ becomes a heightened concern. We require that $\texttt{query}(t | s) = \texttt{query}(s | t)$ for all $(s,t) \in E$. That is, the adjacency oracles corresponding to $s$ and $t$ have the same output regarding whether $(s,t)$ is an edge in $H$.

\subsection{}

==> techoverview.tex <==
\section{Technical Overview}

\gbnoteinline{not currently sure if we want this. tbd}
